Anisotropic analysis of VEM for time-harmonic Maxwell equations in inhomogeneous media with low regularity

It has been extensively studied in the literature that solving Maxwell equations is very sensitive to the mesh structure, space conformity and solution regularity. Roughly speaking, for almost all the methods in the literature, optimal convergence for low-regularity solutions heavily relies on conforming spaces and highly-regular simplicial meshes. This can be a significant limitation for many popular methods based on polytopal meshes in the case of inhomogeneous media, as the discontinuity of electromagnetic parameters can lead to quite low regularity of solutions near media interfaces, and potentially worsened by geometric singularities, making many popular methods based on broken spaces, non-conforming or polytopal meshes particularly challenging to apply. In this article, we present a virtual element method for solving an indefinite time-harmonic Maxwell equation in 2D inhomogeneous media with quite arbitrary polytopal meshes, and the media interface is allowed to have geometric singularity to cause low regularity. There are two key novelties: (i) the proposed method is theoretically guaranteed to achieve robust optimal convergence for solutions with merely $\mathbf{H}^{\theta}$ regularity, $\theta\in(1/2,1]$; (ii) the polytopal element shape can be highly anisotropic and shrinking, and an explicit formula is established to describe the relationship between the shape regularity and solution regularity. Extensive numerical experiments will be given to demonstrate the effectiveness of the proposed method.

==> Makefile <==

all: Helmholtz2D.pdf \

Helmholtz2D.pdf: Helmholtz2D.tex
	pdflatex -shell-escape Helmholtz2D.tex
	bibtex Helmholtz2D.aux
	pdflatex -shell-escape Helmholtz2D.tex
	pdflatex -shell-escape Helmholtz2D.tex
	evince Helmholtz2D.pdf&


.PHONY:clean  
clean:
	-rm -fr *.ps *.dvi *.aux *.toc *.idx *.ind *.ilg *.log *.out *~ *.tid *.tms *.bak *.blg *.bbl *.gz *.snm *.nav _minted*


